Satisfied, Not Solving: Wireheading of Bounded Homeostatic Rewards in Reinforcement Learning

Bounded intrinsic rewards are often assumed to be safe from exploitation: if a signal can yield at most a fixed amount, gaming it should not pay. We test this for a homeostatic satiation reward, in which needs build up and relieving them is rewarding, and give the agent a cheap action that resets its needs. In MiniGrid DoorKey-8x8, PPO agents with this action solved 2 of 80 seeds, against 71 of 80 on the same seeds without it; in KeyCorridorS3R1, 0 of 20 against 20 of 20. Their policies stayed near uniform. The reward does not ask for this: a telescoping argument caps any policy's satiation return at the needs' starting drive, and a post-hoc computation shows that, at every growth rate we trained, a solving trajectory beats that cap on all sampled layouts. In DoorKey with advantage normalization on, a satisfaction signal the agent could fill itself was worse than none (11 of 20 solved with task reward alone, 1 of 20 with the tamperable signal), and a per-press cost of 0.1 restored the task in every seed. Farming of positive reward cycles appeared in DoorKey but not persistently in KeyCorridorS3R1. All predictions were pre-registered, and hash-locked from round 3 on; 9 of our 23 hypotheses were not supported, and we report each.

==> numbers.tex <==
% Generated by paper/scripts/make_numbers.py from paper/data. Do not edit by hand.
\makeatletter
\@namedef{val@cons.rows}{94}
\@namedef{val@cons.hits}{60}
\@namedef{val@cons.misses}{32}
\@namedef{val@cons.unres}{2}
\@namedef{val@cons.ncorr}{13}
\@namedef{val@r4.solve.B1}{1/20}
\@namedef{val@r4.farm.B1}{6/20}
\@namedef{val@r4.prolong.B1}{13/20}
\@namedef{val@r4.solve.B2}{0/20}
\@namedef{val@r4.farm.B2}{20/20}
\@namedef{val@r4.prolong.B2}{0/20}
\@namedef{val@r4.solve.B3}{1/20}
\@namedef{val@r4.farm.B3}{5/20}
\@namedef{val@r4.prolong.B3}{14/20}
\@namedef{val@r4.solve.B4}{0/20}
\@namedef{val@r4.farm.B4}{18/20}
\@namedef{val@r4.prolong.B4}{2/20}
\@namedef{val@r4.solve.B5}{11/20}
\@namedef{val@r4.farm.B5}{9/20}
\@namedef{val@r4.prolong.B5}{0/20}
\@namedef{val@r4.solve.B6}{20/20}
\@namedef{val@r4.farm.B6}{0/20}
\@namedef{val@r4.prolong.B6}{0/20}
\@namedef{val@r4.solve.B7}{20/20}
\@namedef{val@r4.farm.B7}{0/20}
\@namedef{val@r4.prolong.B7}{0/20}
\@namedef{val@r4.solve.B8}{0/20}
\@namedef{val@r4.farm.B8}{20/20}
\@namedef{val@r4.prolong.B8}{0/20}
\@namedef{val@r4.solve.A1a}{20/20}
\@namedef{val@r4.farm.A1a}{0/20}
\@namedef{val@r4.prolong.A1a}{0/20}
\@namedef{val@r4.solve.A1b}{20/20}
\@namedef{val@r4.farm.A1b}{0/20}
\@namedef{val@r4.prolong.A1b}{0/20}
\@namedef{val@r4.solve.A1c}{20/20}
\@namedef{val@r4.farm.A1c}{0/20}
\@namedef{val@r4.prolong.A1c}{0/20}
\@namedef{val@r4.solve.A2a}{11/20}
\@namedef{val@r4.farm.A2a}{7/20}
\@namedef{val@r4.prolong.A2a}{2/20}
\@namedef{val@r4.solve.A2b}{0/20}
\@namedef{val@r4.farm.A2b}{20/20}
\@namedef{val@r4.prolong.A2b}{0/20}
\@namedef{val@r4.solve.A2c}{17/20}
\@namedef{val@r4.farm.A2c}{2/20}
\@namedef{val@r4.prolong.A2c}{0/20}
\@namedef{val@r4.solve.on}{2/80}
\@namedef{val@r4.solve.off}{71/80}
\@namedef{val@p.PB2-B1}{$1.5\times10^{-10}$}
\@namedef{val@ph.PB2-B1}{$2.3\times10^{-9}$}
\@namedef{val@p.PB2-B2}{$7.3\times10^{-12}$}
\@namedef{val@ph.PB2-B2}{$1.2\times10^{-10}$}
\@namedef{val@p.PB2-B3}{0.00062}
\@namedef{val@ph.PB2-B3}{0.006}
\@namedef{val@p.PB2-B4}{$7.3\times10^{-12}$}
\@namedef{val@ph.PB2-B4}{$1.2\times10^{-10}$}
\@namedef{val@p.PB4}{0.00061}
\@namedef{val@ph.PB4}{0.006}
\@namedef{val@p.PB3-B1}{1.000}
\@namedef{val@ph.PB3-B1}{1.000}
\@namedef{val@p.PB3-B3}{1.000}
\@namedef{val@ph.PB3-B3}{1.000}
\@namedef{val@p.A1-P1}{0.708}
\@namedef{val@ph.A1-P1}{1.000}
\@namedef{val@p.A1-P2}{0.744}
\@namedef{val@ph.A1-P2}{1.000}
\@namedef{val@p.A2-P1}{0.00018}
\@namedef{val@ph.A2-P1}{0.002}
\@namedef{val@p.A2-P2}{$5\times10^{-6}$}
\@namedef{val@ph.A2-P2}{$6.5\times10^{-5}$}
\@namedef{val@p.A2-P3}{0.002}
\@namedef{val@ph.A2-P3}{0.015}
\@namedef{val@p.A2-P4}{$5\times10^{-6}$}
\@namedef{val@ph.A2-P4}{$6.5\times10^{-5}$}
\@namedef{val@p.A2-P5}{0.041}
\@namedef{val@ph.A2-P5}{0.247}
\@namedef{val@p.A2-P6}{$1.3\times10^{-8}$}
\@namedef{val@ph.A2-P6}{$1.8\times10^{-7}$}
\@namedef{val@p.A2-P7}{0.371}
\@namedef{val@ph.A2-P7}{1.000}
\@namedef{val@p.A2-P8}{0.002}
\@namedef{val@ph.A2-P8}{0.013}
\@namedef{val@p.PB1-pooled}{$8.3\times10^{-25}$}
\@namedef{val@p.PB5}{$9.5\times10^{-7}$}
\@namedef{val@r4.tamperers.on}{80/80}
\@namedef{val@r4.loopers.on}{80/80}
\@namedef{val@r4.solverseed.B1}{48}
\@namedef{val@r4.solverseed.B3}{48}
\@namedef{val@r4.intr.on.lo}{0.71}
\@namedef{val@r4.intr.on.hi}{0.74}
\@namedef{val@r4.intr.off.lo}{0.56}
\@namedef{val@r4.intr.off.hi}{0.74}
\@namedef{val@r4.key.on.lo}{73}
\@namedef{val@r4.key.on.hi}{92}
\@namedef{val@r4.door.on.lo}{14}
\@namedef{val@r4.door.on.hi}{17}
\@namedef{val@r4.len.on.lo}{607}
\@namedef{val@r4.len.on.hi}{635}
\@namedef{val@r4.B8.pick}{297}
\@namedef{val@r4.B8.intr}{77}
\@namedef{val@d.doneshare.B1}{0.061}
\@namedef{val@d.doneshare.B2}{0.096}
\@namedef{val@d.doneshare.B3}{0.270}
\@namedef{val@d.doneshare.B4}{0.189}
\@namedef{val@d.doneshare.A1b}{0.000}
\@namedef{val@d.doneshare.B7}{0.081}
\@namedef{val@d.doneshare.B5}{0.000}
\@namedef{val@d.doneshare.B6}{0.019}
\@namedef{val@tr.disc.lo}{0.694}
\@namedef{val@tr.disc.hi}{0.722}
\@namedef{val@tr.total.lo}{0.694}
\@namedef{val@tr.total.hi}{0.723}
\@namedef{val@tr.drive.lo}{0.018}
\@namedef{val@tr.drive.hi}{0.043}
\@namedef{val@tr.success.lo}{0.000}
\@namedef{val@tr.success.hi}{0.022}
\@namedef{val@tr.npol}{80}
\@namedef{val@tr.presscheck.max}{0.007}
\@namedef{val@tr.cappct.lo}{93}
\@namedef{val@tr.cappct.hi}{96}
\@namedef{val@d.done200k.B1}{0.25}
\@namedef{val@d.ent200k.B1}{1.86}
\@namedef{val@d.done200k.B2}{0.16}
\@namedef{val@d.ent200k.B2}{1.94}
\@namedef{val@d.done200k.B3}{0.71}
\@namedef{val@d.ent200k.B3}{1.02}
\@namedef{val@d.done200k.B4}{0.27}
\@namedef{val@d.ent200k.B4}{1.90}
\@namedef{val@uniform.press}{0.143}
\@namedef{val@uniform.press.ep}{91}
\@namedef{val@ln7}{1.946}
\@namedef{val@d2.on.B1}{1.878}
\@namedef{val@d2.off.A1b}{0.067}
\@namedef{val@d2.on.B2}{1.935}
\@namedef{val@d2.off.B7}{1.138}
\@namedef{val@d2.on.B3}{1.844}
\@namedef{val@d2.off.B5}{0.290}
\@namedef{val@d2.on.B4}{1.934}
\@namedef{val@d2.off.B6}{0.598}
\@namedef{val@p.D2}{$7.3\times10^{-12}$}
\@namedef{val@ph.D2.max}{$1.5\times10^{-10}$}
\@namedef{val@d1.never}{1/80}
\@namedef{val@d1.lost}{77/80}
\@namedef{val@d1.kept}{2/80}
\@namedef{val@d1.declined}{7/77}
\@namedef{val@d1.declined.pct}{9}
\@namedef{val@d1.firstgoal.median}{27,344}
\@namedef{val@d1.firstgoal.max}{1,187,264}
\@namedef{val@d3.rise}{7/7}
\@namedef{val@d3.n}{7}
\@namedef{val@d3.norise}{17}
\@namedef{val@d3.nodecline}{56}
\@namedef{val@p.D3}{0.008}
\@namedef{val@r5.solve.A1}{11/20}
\@namedef{val@r5.ci.A1}{[0.32, 0.77]}
\@namedef{val@r5.auc.A1}{0.438}
\@namedef{val@r5.farm.A1}{0/20}
\@namedef{val@r5.tamperers.A1}{9/20}
\@namedef{val@r5.solve.A2}{0/20}
\@namedef{val@r5.ci.A2}{[0.00, 0.17]}
\@namedef{val@r5.auc.A2}{0.025}
\@namedef{val@r5.farm.A2}{0/20}
\@namedef{val@r5.tamperers.A2}{20/20}
\@namedef{val@r5.solve.B9}{3/20}
\@namedef{val@r5.ci.B9}{[0.03, 0.38]}
\@namedef{val@r5.auc.B9}{0.147}
\@namedef{val@r5.farm.B9}{8/20}
\@namedef{val@r5.tamperers.B9}{19/20}
\@namedef{val@r5.solve.B10}{20/20}
\@namedef{val@r5.ci.B10}{[0.83, 1.00]}
\@namedef{val@r5.auc.B10}{0.601}
\@namedef{val@r5.farm.B10}{0/20}
\@namedef{val@r5.tamperers.B10}{7/20}
\@namedef{val@r5.solve.B11}{20/20}
\@namedef{val@r5.ci.B11}{[0.83, 1.00]}
\@namedef{val@r5.auc.B11}{0.816}
\@namedef{val@r5.farm.B11}{0/20}
\@namedef{val@r5.tamperers.B11}{0/20}
\@namedef{val@r5.solve.C1}{20/20}
\@namedef{val@r5.ci.C1}{[0.83, 1.00]}
\@namedef{val@r5.auc.C1}{0.958}
\@namedef{val@r5.farm.C1}{0/20}
\@namedef{val@r5.tamperers.C1}{0/20}
\@namedef{val@r5.solve.C2}{20/20}
\@namedef{val@r5.ci.C2}{[0.83, 1.00]}
\@namedef{val@r5.auc.C2}{0.961}
\@namedef{val@r5.farm.C2}{0/20}
\@namedef{val@r5.tamperers.C2}{0/20}
\@namedef{val@r5.solve.C3}{20/20}
\@namedef{val@r5.ci.C3}{[0.83, 1.00]}
\@namedef{val@r5.auc.C3}{0.932}
\@namedef{val@r5.farm.C3}{0/20}
\@namedef{val@r5.tamperers.C3}{0/20}
\@namedef{val@r5.solve.C4}{20/20}
\@namedef{val@r5.ci.C4}{[0.83, 1.00]}
\@namedef{val@r5.auc.C4}{0.929}
\@namedef{val@r5.farm.C4}{0/20}
\@namedef{val@r5.tamperers.C4}{0/20}
\@namedef{val@r5.solve.C5}{0/20}
\@namedef{val@r5.ci.C5}{[0.00, 0.17]}
\@namedef{val@r5.auc.C5}{0.002}
\@namedef{val@r5.farm.C5}{0/20}
\@namedef{val@r5.tamperers.C5}{20/20}
\@namedef{val@r5.solve.C6}{20/20}
\@namedef{val@r5.ci.C6}{[0.83, 1.00]}
\@namedef{val@r5.auc.C6}{0.875}
\@namedef{val@r5.farm.C6}{0/20}
\@namedef{val@r5.tamperers.C6}{0/20}
\@namedef{val@r5.solve.r4B1}{1/20}
\@namedef{val@r5.ci.r4B1}{[0.00, 0.25]}
\@namedef{val@r5.auc.r4B1}{0.042}
\@namedef{val@r5.farm.r4B1}{6/20}
\@namedef{val@r5.tamperers.r4B1}{20/20}
\@namedef{val@r5.solve.r4B2}{0/20}
\@namedef{val@r5.ci.r4B2}{[0.00, 0.17]}
\@namedef{val@r5.auc.r4B2}{0.022}
\@namedef{val@r5.farm.r4B2}{20/20}
\@namedef{val@r5.tamperers.r4B2}{20/20}
\@namedef{val@r5.solve.r4B3}{1/20}
\@namedef{val@r5.ci.r4B3}{[0.00, 0.25]}
\@namedef{val@r5.auc.r4B3}{0.036}
\@namedef{val@r5.farm.r4B3}{5/20}
\@namedef{val@r5.tamperers.r4B3}{20/20}
\@namedef{val@r5.solve.r4A1b}{20/20}
\@namedef{val@r5.ci.r4A1b}{[0.83, 1.00]}
\@namedef{val@r5.auc.r4A1b}{0.901}
\@namedef{val@r5.farm.r4A1b}{0/20}
\@namedef{val@r5.tamperers.r4A1b}{0/20}
\@namedef{val@r5.auc.B1B3}{0.039}
\@namedef{val@r5.solve.B1B3}{2/40}
\@namedef{val@p.A-P1}{0.00062}
\@namedef{val@ph.A-P1}{0.004}
\@namedef{val@p.A-P1m}{$7.8\times10^{-6}$}
\@namedef{val@ph.A-P1m}{$7\times10^{-5}$}
\@namedef{val@p.A-P2}{1.000}
\@namedef{val@ph.A-P2}{1.000}
\@namedef{val@p.A-P2m}{0.005}
\@namedef{val@ph.A-P2m}{0.028}
\@namedef{val@p.A-P3}{$2.6\times10^{-5}$}
\@namedef{val@ph.A-P3}{0.00021}
\@namedef{val@p.A-P3m}{$5\times10^{-6}$}
\@namedef{val@ph.A-P3m}{$6\times10^{-5}$}
\@namedef{val@p.B-JTp}{$5\times10^{-6}$}
\@namedef{val@ph.B-JTp}{$6\times10^{-5}$}
\@namedef{val@p.B-JTs}{$5\times10^{-6}$}
\@namedef{val@ph.B-JTs}{$6\times10^{-5}$}
\@namedef{val@p.B-F-B9-vsB1}{0.302}
\@namedef{val@p.B-F-B9-vsA1b}{$1.3\times10^{-8}$}
\@namedef{val@ph.B-F-B9-vsA1b}{$1.7\times10^{-7}$}
\@namedef{val@p.B-F-B10-vsB1}{$1.5\times10^{-10}$}
\@namedef{val@p.B-F-B10-vsA1b}{1.000}
\@namedef{val@ph.B-F-B10-vsA1b}{1.000}
\@namedef{val@p.B-F-B11-vsB1}{$1.5\times10^{-10}$}
\@namedef{val@ph.B-F-B11-vsB1}{$2.1\times10^{-9}$}
\@namedef{val@p.B-F-B11-vsA1b}{1.000}
\@namedef{val@p.C-P1}{1.000}
\@namedef{val@ph.C-P1}{1.000}
\@namedef{val@p.C-P2}{1.000}
\@namedef{val@ph.C-P2}{1.000}
\@namedef{val@p.C-P3}{$7.3\times10^{-12}$}
\@namedef{val@ph.C-P3}{$1.5\times10^{-10}$}
\@namedef{val@p.C-P4}{$7.3\times10^{-12}$}
\@namedef{val@ph.C-P4}{$1.5\times10^{-10}$}
\@namedef{val@exp.B-L-B9-presses}{30}
\@namedef{val@rng.B-L-B9-presses}{12--45}
\@namedef{val@obs.B-L-B9-presses}{27.13}
\@namedef{val@exp.B-L-B9-tamperers}{20/20}
\@namedef{val@rng.B-L-B9-tamperers}{16--20}
\@namedef{val@obs.B-L-B9-tamperers}{19/20}
\@namedef{val@exp.B-L-B9-solves}{1/20}
\@namedef{val@rng.B-L-B9-solves}{0--5}
\@namedef{val@obs.B-L-B9-solves}{3/20}
\@namedef{val@exp.B-L-B10-presses}{8}
\@namedef{val@rng.B-L-B10-presses}{1--30}
\@namedef{val@obs.B-L-B10-presses}{0.36}
\@namedef{val@exp.B-L-B10-tamperers}{17/20}
\@namedef{val@rng.B-L-B10-tamperers}{10--20}
\@namedef{val@obs.B-L-B10-tamperers}{7/20}
\@namedef{val@exp.B-L-B10-solves}{3/20}
\@namedef{val@rng.B-L-B10-solves}{0--10}
\@namedef{val@obs.B-L-B10-solves}{20/20}
\@namedef{val@exp.B-L-B11-presses}{0.2}
\@namedef{val@rng.B-L-B11-presses}{0--3}
\@namedef{val@obs.B-L-B11-presses}{0.00}
\@namedef{val@exp.B-L-B11-tamperers}{3/20}
\@namedef{val@rng.B-L-B11-tamperers}{0--10}
\@namedef{val@obs.B-L-B11-tamperers}{0/20}
\@namedef{val@exp.B-L-B11-solves}{17/20}
\@namedef{val@rng.B-L-B11-solves}{11--20}
\@namedef{val@obs.B-L-B11-solves}{20/20}
\@namedef{val@pps.B1}{0.061}
\@namedef{val@pps.iqr.B1}{[0.060, 0.063]}
\@namedef{val@len.B1}{635}
\@namedef{val@pps.B9}{0.043}
\@namedef{val@pps.iqr.B9}{[0.042, 0.044]}
\@namedef{val@len.B9}{627}
\@namedef{val@pps.B10}{0.010}
\@namedef{val@pps.iqr.B10}{[0.001, 0.020]}
\@namedef{val@len.B10}{35}
\@namedef{val@pps.B11}{0.000}
\@namedef{val@pps.iqr.B11}{[0.000, 0.000]}
\@namedef{val@len.B11}{22}
\@namedef{val@pps.A1b}{0.000}
\@namedef{val@pps.iqr.A1b}{[0.000, 0.000]}
\@namedef{val@len.A1b}{20}
\@namedef{val@s0.160.tamper}{0.0114}
\@namedef{val@s0.160.notamper}{0.0128}
\@namedef{val@s0.160.adv}{0.012}
\@namedef{val@s0.40.tamper}{0.035}
\@namedef{val@s0.40.notamper}{0.0351}
\@namedef{val@s0.40.adv}{0.048}
\@namedef{val@r5.fs.C1}{137k}
\@namedef{val@r5.fs.C2}{138k}
\@namedef{val@r5.fs.C3}{202k}
\@namedef{val@r5.fs.C6}{258k}
\@namedef{val@kc.peak.C1}{8.0}
\@namedef{val@kc.peakmax.C1}{9.9}
\@namedef{val@kc.peak.C2}{12.4}
\@namedef{val@kc.peakmax.C2}{14.4}
\@namedef{val@kc.peak.C3}{28.3}
\@namedef{val@kc.peakmax.C3}{48.5}
\@namedef{val@kc.peak.C4}{21.7}
\@namedef{val@kc.peakmax.C4}{26.8}
\@namedef{val@kc.peak.C5}{2.0}
\@namedef{val@kc.peakmax.C5}{2.4}
\@namedef{val@kc.peak.C6}{5.7}
\@namedef{val@kc.peakmax.C6}{9.6}
\@namedef{val@kc.final.lo}{1.0}
\@namedef{val@kc.final.hi}{1.7}
\@namedef{val@kc.C5.pick}{0.15}
\@namedef{val@kc.overrepeat}{1/80}
\@namedef{val@kc.final.max}{5.16}
\@namedef{val@kc.C5.entropy}{1.85}
\@namedef{val@exp.C3.farm}{12/20}
\@namedef{val@exp.C3.range}{5--20}
\@namedef{val@exp.C2.farm}{4/20}
\@namedef{val@exp.C5.solve}{6/20}
\@namedef{val@r5.A2.presses.ep}{91}
\@namedef{val@r5.A2.pick}{5.69}
\@namedef{val@holm.r4}{17}
\@namedef{val@holm.r5}{20}
\@namedef{val@r4.fs.A1a}{221,640}
\@namedef{val@r4.sl.A1a}{19.6}
\@namedef{val@r4.fs.A1b}{311,832}
\@namedef{val@r4.sl.A1b}{20.3}
\@namedef{val@r4.fs.A1c}{283,424}
\@namedef{val@r4.sl.A1c}{19.7}
\@namedef{val@r4.curve8.A2a}{0.387}
\@namedef{val@r4.curve16.A2a}{0.328}
\@namedef{val@r4.solve16.A2a}{6/20}
\@namedef{val@r4.curve8.A2b}{0.060}
\@namedef{val@r4.curve16.A2b}{0.011}
\@namedef{val@r4.solve16.A2b}{0/20}
\@namedef{val@r4.curve8.A2c}{0.702}
\@namedef{val@r4.curve16.A2c}{0.579}
\@namedef{val@r4.solve16.A2c}{8/20}
\@namedef{val@a2.coef.640}{1.226}
\@namedef{val@a2.coef.160}{7.355}
\@namedef{val@r3.farm.R1}{4/20}
\@namedef{val@r3.solve.R1}{16/20}
\@namedef{val@r3.farm.R2}{18/20}
\@namedef{val@r3.solve.R2}{2/20}
\@namedef{val@r3.farm.R3}{6/20}
\@namedef{val@r3.solve.R3}{14/20}
\@namedef{val@r3.farm.R4}{9/20}
\@namedef{val@r3.solve.R4}{11/20}
\@namedef{val@r3.farm.R5}{12/20}
\@namedef{val@r3.solve.R5}{8/20}
\@namedef{val@r3.farm.R6}{0/20}
\@namedef{val@r3.solve.R6}{20/20}
\@namedef{val@r3.farm.R7}{0/20}
\@namedef{val@r3.solve.R7}{20/20}
\@namedef{val@r3.farm.R8}{0/20}
\@namedef{val@r3.solve.R8}{20/20}
\@namedef{val@r3.farm.R9}{10/20}
\@namedef{val@r3.solve.R9}{10/20}
\@namedef{val@r3.farm.R10}{0/20}
\@namedef{val@r3.solve.R10}{20/20}
\@namedef{val@r3.normon.total}{27/60}
\@namedef{val@r3.normoff.total}{0/60}
\@namedef{val@p.R1<R4}{0.088}
\@namedef{val@p.R2>R4}{0.003}
\@namedef{val@p.R8>R6}{1.000}
\@namedef{val@p.R9<R4}{0.736}
\@namedef{val@exp.R7.range}{5--15}
\@namedef{val@exp.R8.range}{11--20}
\@namedef{val@exp.R9.range}{0--4}
\@namedef{val@r2.farm.N1}{7/10}
\@namedef{val@r2.rescore.N1}{6/10}
\@namedef{val@r2.E.N1}{0.764}
\@namedef{val@r2.range.N1}{2--8}
\@namedef{val@r2.farm.N2}{7/10}
\@namedef{val@r2.rescore.N2}{7/10}
\@namedef{val@r2.E.N2}{0.281}
\@namedef{val@r2.range.N2}{0--2}
\@namedef{val@r2.farm.N3}{0/10}
\@namedef{val@r2.rescore.N3}{0/10}
\@namedef{val@r2.E.N3}{0.593}
\@namedef{val@r2.range.N3}{1--4}
\@namedef{val@r2.farm.N4}{0/10}
\@namedef{val@r2.rescore.N4}{0/10}
\@namedef{val@r2.E.N4}{0.764}
\@namedef{val@r2.range.N4}{2--8}
\@namedef{val@r2.farm.N5}{3/10}
\@namedef{val@r2.rescore.N5}{3/10}
\@namedef{val@r2.E.N5}{0.382}
\@namedef{val@r2.range.N5}{0--1}
\@namedef{val@r2.farm.N6}{10/10}
\@namedef{val@r2.rescore.N6}{9/10}
\@namedef{val@r2.E.N6}{0.87}
\@namedef{val@r2.range.N6}{6--10}
\@namedef{val@r2.farm.payonce}{10/10}
\@namedef{val@p.N2<N1}{0.686}
\@namedef{val@p.N5<N4}{1.000}
\@namedef{val@p.N6>N3}{$5.4\times10^{-6}$}
\@namedef{val@r2.slope}{1.06}
\@namedef{val@p.r2logistic}{0.193}
\@namedef{val@n6.rint.lo}{$-$1.54}
\@namedef{val@n6.rint.hi}{$-$1.27}
\@namedef{val@n6.pick.lo}{137}
\@namedef{val@n6.pick.hi}{184}
\@namedef{val@n6.pdshare.lo}{48}
\@namedef{val@n6.pdshare.hi}{63}
\@namedef{val@n6.nfarm}{9}
\@namedef{val@n6.need.explore.lo}{0.90}
\@namedef{val@n6.need.explore.hi}{0.96}
\@namedef{val@n6.need.explore}{0.90--0.96}
\@namedef{val@n6.need.grasp.lo}{0.10}
\@namedef{val@n6.need.grasp.hi}{0.33}
\@namedef{val@n6.need.grasp}{0.10--0.33}
\@namedef{val@n6.need.open.lo}{1.00}
\@namedef{val@n6.need.open.hi}{1.00}
\@namedef{val@n6.need.open}{1.00}
\@namedef{val@acct.groups}{23}
\@namedef{val@acct.supported}{14}
\@namedef{val@acct.notsupported}{9}
\@namedef{val@race.P1.undet}{21/30}
\@namedef{val@race.P2}{60/60}
\@namedef{val@p.race.P2}{$8.7\times10^{-19}$}
\@namedef{val@vi.maxreach}{1/4}
\@namedef{val@vi.cycles}{1/2}
\@namedef{val@vi.steps}{11}
\@namedef{val@b0.160.tampers}{1}
\@namedef{val@b0.160.at}{0}
\@namedef{val@b0.160.steps}{12}
\@namedef{val@b0.40.tampers}{2}
\@namedef{val@b0.40.at}{0, 11}
\@namedef{val@b0.40.steps}{13}
\@namedef{val@bc.layouts}{200}
\@namedef{val@bc.dk.len.min}{9}
\@namedef{val@bc.dk.len.median}{17}
\@namedef{val@bc.dk.len.max}{26}
\@namedef{val@bc.kc.len.min}{14}
\@namedef{val@bc.kc.len.median}{15}
\@namedef{val@bc.kc.len.max}{15}
\@namedef{val@bc.dk20.short.le}{35}
\@namedef{val@bc.dk20.short.le.u}{20}
\@namedef{val@bc.dk20.short.min}{0.371}
\@namedef{val@bc.dk20.tamper.le}{27}
\@namedef{val@bc.dk20.rich.min}{0.966}
\@namedef{val@bc.dk20.rich.umin}{1.212}
\@namedef{val@bc.dk20.rich.regrab}{199}
\@namedef{val@bc.dk.simplemin.not20}{0.989}
\@namedef{val@bc.tamperfam.min}{1.462}
\@namedef{val@bc.rich.min.all}{0.966}
\@namedef{val@bs.nfarm}{9}
\@namedef{val@bs.mean}{$-$0.936}
\@namedef{val@bs.maxns}{$-$0.535}
\@namedef{val@bs.maxns.u}{$-$1.012}
\@namedef{val@bs.nns}{1,749}
\@namedef{val@bs.beat}{0}
\@namedef{val@bs.best.min}{0.966}
\@namedef{val@bs.best.median}{1.244}
\@namedef{val@bs.solveeps}{52}
\@namedef{val@bs.solverseed.rate}{0.995}
\@namedef{val@bs.n6seed6.rate}{0.26}
\@namedef{val@compute.runs.r25}{43}
\@namedef{val@compute.hours.r25}{12.8}
\@namedef{val@compute.runs.r1}{14}
\@namedef{val@compute.hours.r1}{3.0}
\@namedef{val@hash.r3}{b5e845c978ec96c2746eb81098c0bea3bf8dc14a1dc174e4f77844352b621ae7}
\@namedef{val@hash.r4}{79fdfed000d5e6f892d9201cadd970808cf3b0949e4b3e3d925be9839800faa1}
\@namedef{val@hash.r4a}{72b77be693b9d493e756b23f89aadb35d6934965d5c0633d4681fc8422c0e6f5}
\@namedef{val@hash.r5}{0298bbc79c323e4613e56a29be0257a6c7c3ad764cbb056902159292bcbcda0d}
\@namedef{val@hash.r5a}{1d99028349683b3b85bd204802b614bfb3a38fa30db3d24fbb19eda7c2790a4f}
\@namedef{val@lock.r3}{2026-10-26 15:17:42}
\@namedef{val@lock.r4}{2026-10-26 19:23:42}
\@namedef{val@lock.r5}{2026-10-27 04:34:11}
\@namedef{val@ver.torch}{2.14.1}
\@namedef{val@ver.gymnasium}{1.4.0}
\@namedef{val@ver.minigrid}{3.2.0}
\@namedef{val@ver.numpy}{2.5.4}
\@namedef{val@ver.python}{3.12.12}
\@namedef{val@r4.solve.B1.of}{1 of 20}
\@namedef{val@r4.farm.B1.of}{6 of 20}
\@namedef{val@r4.prolong.B1.of}{13 of 20}
\@namedef{val@r4.solve.B2.of}{0 of 20}
\@namedef{val@r4.farm.B2.of}{20 of 20}
\@namedef{val@r4.prolong.B2.of}{0 of 20}
\@namedef{val@r4.solve.B3.of}{1 of 20}
\@namedef{val@r4.farm.B3.of}{5 of 20}
\@namedef{val@r4.prolong.B3.of}{14 of 20}
\@namedef{val@r4.solve.B4.of}{0 of 20}
\@namedef{val@r4.farm.B4.of}{18 of 20}
\@namedef{val@r4.prolong.B4.of}{2 of 20}
\@namedef{val@r4.solve.B5.of}{11 of 20}
\@namedef{val@r4.farm.B5.of}{9 of 20}
\@namedef{val@r4.prolong.B5.of}{0 of 20}
\@namedef{val@r4.solve.B6.of}{20 of 20}
\@namedef{val@r4.farm.B6.of}{0 of 20}
\@namedef{val@r4.prolong.B6.of}{0 of 20}
\@namedef{val@r4.solve.B7.of}{20 of 20}
\@namedef{val@r4.farm.B7.of}{0 of 20}
\@namedef{val@r4.prolong.B7.of}{0 of 20}
\@namedef{val@r4.solve.B8.of}{0 of 20}
\@namedef{val@r4.farm.B8.of}{20 of 20}
\@namedef{val@r4.prolong.B8.of}{0 of 20}
\@namedef{val@r4.solve.A1a.of}{20 of 20}
\@namedef{val@r4.farm.A1a.of}{0 of 20}
\@namedef{val@r4.prolong.A1a.of}{0 of 20}
\@namedef{val@r4.solve.A1b.of}{20 of 20}
\@namedef{val@r4.farm.A1b.of}{0 of 20}
\@namedef{val@r4.prolong.A1b.of}{0 of 20}
\@namedef{val@r4.solve.A1c.of}{20 of 20}
\@namedef{val@r4.farm.A1c.of}{0 of 20}
\@namedef{val@r4.prolong.A1c.of}{0 of 20}
\@namedef{val@r4.solve.A2a.of}{11 of 20}
\@namedef{val@r4.farm.A2a.of}{7 of 20}
\@namedef{val@r4.prolong.A2a.of}{2 of 20}
\@namedef{val@r4.solve.A2b.of}{0 of 20}
\@namedef{val@r4.farm.A2b.of}{20 of 20}
\@namedef{val@r4.prolong.A2b.of}{0 of 20}
\@namedef{val@r4.solve.A2c.of}{17 of 20}
\@namedef{val@r4.farm.A2c.of}{2 of 20}
\@namedef{val@r4.prolong.A2c.of}{0 of 20}
\@namedef{val@r4.solve.on.of}{2 of 80}
\@namedef{val@r4.solve.off.of}{71 of 80}
\@namedef{val@r4.tamperers.on.of}{80 of 80}
\@namedef{val@r4.loopers.on.of}{80 of 80}
\@namedef{val@d1.never.of}{1 of 80}
\@namedef{val@d1.lost.of}{77 of 80}
\@namedef{val@d1.kept.of}{2 of 80}
\@namedef{val@d1.declined.of}{7 of 77}
\@namedef{val@d3.rise.of}{7 of 7}
\@namedef{val@r5.solve.A1.of}{11 of 20}
\@namedef{val@r5.farm.A1.of}{0 of 20}
\@namedef{val@r5.tamperers.A1.of}{9 of 20}
\@namedef{val@r5.solve.A2.of}{0 of 20}
\@namedef{val@r5.farm.A2.of}{0 of 20}
\@namedef{val@r5.tamperers.A2.of}{20 of 20}
\@namedef{val@r5.solve.B9.of}{3 of 20}
\@namedef{val@r5.farm.B9.of}{8 of 20}
\@namedef{val@r5.tamperers.B9.of}{19 of 20}
\@namedef{val@r5.solve.B10.of}{20 of 20}
\@namedef{val@r5.farm.B10.of}{0 of 20}
\@namedef{val@r5.tamperers.B10.of}{7 of 20}
\@namedef{val@r5.solve.B11.of}{20 of 20}
\@namedef{val@r5.farm.B11.of}{0 of 20}
\@namedef{val@r5.tamperers.B11.of}{0 of 20}
\@namedef{val@r5.solve.C1.of}{20 of 20}
\@namedef{val@r5.farm.C1.of}{0 of 20}
\@namedef{val@r5.tamperers.C1.of}{0 of 20}
\@namedef{val@r5.solve.C2.of}{20 of 20}
\@namedef{val@r5.farm.C2.of}{0 of 20}
\@namedef{val@r5.tamperers.C2.of}{0 of 20}
\@namedef{val@r5.solve.C3.of}{20 of 20}
\@namedef{val@r5.farm.C3.of}{0 of 20}
\@namedef{val@r5.tamperers.C3.of}{0 of 20}
\@namedef{val@r5.solve.C4.of}{20 of 20}
\@namedef{val@r5.farm.C4.of}{0 of 20}
\@namedef{val@r5.tamperers.C4.of}{0 of 20}
\@namedef{val@r5.solve.C5.of}{0 of 20}
\@namedef{val@r5.farm.C5.of}{0 of 20}
\@namedef{val@r5.tamperers.C5.of}{20 of 20}
\@namedef{val@r5.solve.C6.of}{20 of 20}
\@namedef{val@r5.farm.C6.of}{0 of 20}
\@namedef{val@r5.tamperers.C6.of}{0 of 20}
\@namedef{val@r5.solve.r4B1.of}{1 of 20}
\@namedef{val@r5.farm.r4B1.of}{6 of 20}
\@namedef{val@r5.tamperers.r4B1.of}{20 of 20}
\@namedef{val@r5.solve.r4B2.of}{0 of 20}
\@namedef{val@r5.farm.r4B2.of}{20 of 20}
\@namedef{val@r5.tamperers.r4B2.of}{20 of 20}
\@namedef{val@r5.solve.r4B3.of}{1 of 20}
\@namedef{val@r5.farm.r4B3.of}{5 of 20}
\@namedef{val@r5.tamperers.r4B3.of}{20 of 20}
\@namedef{val@r5.solve.r4A1b.of}{20 of 20}
\@namedef{val@r5.farm.r4A1b.of}{0 of 20}
\@namedef{val@r5.tamperers.r4A1b.of}{0 of 20}
\@namedef{val@r5.solve.B1B3.of}{2 of 40}
\@namedef{val@exp.B-L-B9-tamperers.of}{20 of 20}
\@namedef{val@obs.B-L-B9-tamperers.of}{19 of 20}
\@namedef{val@exp.B-L-B9-solves.of}{1 of 20}
\@namedef{val@obs.B-L-B9-solves.of}{3 of 20}
\@namedef{val@exp.B-L-B10-tamperers.of}{17 of 20}
\@namedef{val@obs.B-L-B10-tamperers.of}{7 of 20}
\@namedef{val@exp.B-L-B10-solves.of}{3 of 20}
\@namedef{val@obs.B-L-B10-solves.of}{20 of 20}
\@namedef{val@exp.B-L-B11-tamperers.of}{3 of 20}
\@namedef{val@obs.B-L-B11-tamperers.of}{0 of 20}
\@namedef{val@exp.B-L-B11-solves.of}{17 of 20}
\@namedef{val@obs.B-L-B11-solves.of}{20 of 20}
\@namedef{val@kc.overrepeat.of}{1 of 80}
\@namedef{val@exp.C3.farm.of}{12 of 20}
\@namedef{val@exp.C2.farm.of}{4 of 20}
\@namedef{val@exp.C5.solve.of}{6 of 20}
\@namedef{val@r4.solve16.A2a.of}{6 of 20}
\@namedef{val@r4.solve16.A2b.of}{0 of 20}
\@namedef{val@r4.solve16.A2c.of}{8 of 20}
\@namedef{val@r3.farm.R1.of}{4 of 20}
\@namedef{val@r3.solve.R1.of}{16 of 20}
\@namedef{val@r3.farm.R2.of}{18 of 20}
\@namedef{val@r3.solve.R2.of}{2 of 20}
\@namedef{val@r3.farm.R3.of}{6 of 20}
\@namedef{val@r3.solve.R3.of}{14 of 20}
\@namedef{val@r3.farm.R4.of}{9 of 20}
\@namedef{val@r3.solve.R4.of}{11 of 20}
\@namedef{val@r3.farm.R5.of}{12 of 20}
\@namedef{val@r3.solve.R5.of}{8 of 20}
\@namedef{val@r3.farm.R6.of}{0 of 20}
\@namedef{val@r3.solve.R6.of}{20 of 20}
\@namedef{val@r3.farm.R7.of}{0 of 20}
\@namedef{val@r3.solve.R7.of}{20 of 20}
\@namedef{val@r3.farm.R8.of}{0 of 20}
\@namedef{val@r3.solve.R8.of}{20 of 20}
\@namedef{val@r3.farm.R9.of}{10 of 20}
\@namedef{val@r3.solve.R9.of}{10 of 20}
\@namedef{val@r3.farm.R10.of}{0 of 20}
\@namedef{val@r3.solve.R10.of}{20 of 20}
\@namedef{val@r3.normon.total.of}{27 of 60}
\@namedef{val@r3.normoff.total.of}{0 of 60}
\@namedef{val@r2.farm.N1.of}{7 of 10}
\@namedef{val@r2.rescore.N1.of}{6 of 10}
\@namedef{val@r2.farm.N2.of}{7 of 10}
\@namedef{val@r2.rescore.N2.of}{7 of 10}
\@namedef{val@r2.farm.N3.of}{0 of 10}
\@namedef{val@r2.rescore.N3.of}{0 of 10}
\@namedef{val@r2.farm.N4.of}{0 of 10}
\@namedef{val@r2.rescore.N4.of}{0 of 10}
\@namedef{val@r2.farm.N5.of}{3 of 10}
\@namedef{val@r2.rescore.N5.of}{3 of 10}
\@namedef{val@r2.farm.N6.of}{10 of 10}
\@namedef{val@r2.rescore.N6.of}{9 of 10}
\@namedef{val@r2.farm.payonce.of}{10 of 10}
\@namedef{val@race.P1.undet.of}{21 of 30}
\@namedef{val@race.P2.of}{60 of 60}
\@namedef{val@vi.maxreach.of}{1 of 4}
\@namedef{val@vi.cycles.of}{1 of 2}
\makeatother

